Photo-realistic Neural Domain Randomization

Synthetic data is a scalable alternative to manual supervision, but it requires overcoming the sim-to-real domain gap. This discrepancy between virtual and real worlds is addressed by two seemingly opposed approaches: improving the realism of simulation or foregoing realism entirely via domain randomization. In this paper, we show that the recent progress in neural rendering enables a new unified approach we call Photo-realistic Neural Domain Randomization (PNDR). We propose to learn a composition of neural networks that acts as a physics-based ray tracer generating high-quality renderings from scene geometry alone. Our approach is modular, composed of different neural networks for materials, lighting, and rendering, thus enabling randomization of different key image generation components in a differentiable pipeline. Once trained, our method can be combined with other methods and used to generate photo-realistic image augmentations online and significantly more efficiently than via traditional ray-tracing. We demonstrate the usefulness of PNDR through two downstream tasks: 6D object detection and monocular depth estimation. Our experiments show that training with PNDR enables generalization to novel scenes and significantly outperforms the state of the art in terms of real-world transfer.

==> figures_tex/benchmarks.tex <==
\begin{table}[t]
\parbox{.5\linewidth}{
  \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|c|ccc}
    \toprule
    \textbf{Train} & \textbf{Test} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
    \midrule
    \multirow{3}[1]{*}{$HB_2$ - Train} & $HB_2$ - Train & 30.36 & 0.96  & 0.03 \\
          & $HB_2$ - Test  & 26.14 & 0.94  & 0.05 \\
          & $HB_5$ - Test  & 24.14 & 0.92  & 0.06 \\
    \midrule
    \multirow{3}[1]{*}{$HB_5$ - Train} & $HB_5$  - Train & 30.39 & 0.96  & 0.03 \\
          & $HB_5$ - Test  & 26.40 & 0.94  & 0.06 \\
          & $HB_2$ - Test  & 23.72 & 0.92  & 0.07 \\
    \bottomrule
    \end{tabular}%
    }
    % \vspace{2mm}
    \caption{\textbf{PNDR Generalization Performance:} we achieve strong performance not only when applied to a test image of the same scene containing the same objects with different material properties and different poses, but also when applied on a completely different scene.}
  \label{tab:rendering}
}
\hfill
\parbox{.45\linewidth}{
  \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{r|r|ccc}
    \toprule
          & \multicolumn{1}{c|}{\textbf{Modes}} & \textbf{ADD$_{\textbf{AUC}}$} $\uparrow$ & \textbf{IoU}  $\uparrow$ & \textbf{Corr (mm)  $\downarrow$} \\
    \midrule
    \multirow{2}[2]{*}{Material} & \multicolumn{1}{c|}{$A$} & 85.43 & 83.29 & 38.56 \\
          & \multicolumn{1}{c|}{$+S+R$} & 3\%   & 3\%   & 11\% \\
    \midrule
    \multirow{2}[2]{*}{Light} & \multicolumn{1}{c|}{Fixed} & 73.04 & 72.24 & 76.94 \\
          & \multicolumn{1}{c|}{Dynamic} & 21\%  & 19\%  & 55\% \\
    \midrule
    \multirow{2}[2]{*}{Rendering} & \multicolumn{1}{c|}{$D_{dir}$, $G_{dir}$} & 87.09 & 85.55 & 38.42 \\
          & \multicolumn{1}{c|}{+ $D_{ind}$, $G_{ind}$} & 1\%   & 0\%   & 11\% \\
    \midrule
    Full  &       & 88.18 & 85.97 & 34.32 \\
    \bottomrule
    \end{tabular}%
    }
    % \vspace{2mm}
    \caption{\textbf{Ablation:} We analyze the effect of different augmentations on downstream task performance. All methods are trained on the $HB_5$ train set and evaluated on the $HB_5$ test set.}
  \label{tab:ablation}%
}
% \vspace{-6mm}
\end{table}


==> tables/ablation.tex <==
\setlength{\tabcolsep}{6pt}
\begin{table}[!t]
  \centering
  
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{r|r|ccc}
    \toprule
          & \multicolumn{1}{c|}{\textbf{Modes}} & \textbf{ADD$_{\textbf{AUC}}$} $\uparrow$ & \textbf{IoU}  $\uparrow$ & \textbf{Corr (mm)  $\downarrow$} \\
    \midrule
    \multirow{2}[2]{*}{Material} & \multicolumn{1}{c|}{$A$} & 85.43 & 83.29 & 38.56 \\
          & \multicolumn{1}{c|}{$+S+R$} & 3\%   & 3\%   & 11\% \\
    \midrule
    \multirow{2}[2]{*}{Light} & \multicolumn{1}{c|}{Fixed} & 73.04 & 72.24 & 76.94 \\
          & \multicolumn{1}{c|}{Dynamic} & 21\%  & 19\%  & 55\% \\
    \midrule
    \multirow{2}[2]{*}{Rendering} & \multicolumn{1}{c|}{$D_{dir}$, $G_{dir}$} & 87.09 & 85.55 & 38.42 \\
          & \multicolumn{1}{c|}{+ $D_{ind}$, $G_{ind}$} & 1\%   & 0\%   & 11\% \\
    \midrule
    Full  &       & 88.18 & 85.97 & 34.32 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{Ablation:} We analyze the effect of different augmentations on downstream task performance. All methods are trained on the $HB_5$ train set and evaluated on the $HB_5$ test set.}
  \label{tab:ablation}%
%   \vspace*{-2mm}
\end{table}%

% ADD$_{\text{AUC}}$

==> tables/rendering.tex <==
\setlength{\tabcolsep}{6pt}
\begin{table}[t]
  \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|c|ccc}
    \toprule
    \textbf{Train} & \textbf{Test} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} \\
    \midrule
    \multirow{3}[1]{*}{$HB_2$ - Train} & $HB_2$ - Train & 30.36 & 0.96  & 0.03 \\
          & $HB_2$ - Test  & 26.14 & 0.94  & 0.05 \\
          & $HB_5$ - Test  & 24.14 & 0.92  & 0.06 \\
    \midrule
    \multirow{3}[1]{*}{$HB_5$ - Train} & $HB_5$  - Train & 30.39 & 0.96  & 0.03 \\
          & $HB_5$ - Test  & 26.40 & 0.94  & 0.06 \\
          & $HB_2$ - Test  & 23.72 & 0.92  & 0.07 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{\textbf{PNDR Generalization Performance:} we achieve strong performance not only when applied to a test image of the same scene containing the same objects with different material properties and different poses, but also when applied on a completely different scene.}
  \label{tab:rendering}
% \vspace{-6mm}
\end{table}%
